Multi-Robot Relative Pose Estimation and IMU Preintegration Using Passive UWB Transceivers

Ultra-wideband (UWB) systems are becoming increasingly popular as a means of inter-robot ranging and communication. A major constraint associated with UWB is that only one pair of UWB transceivers can range at a time to avoid interference, hence hindering the scalability of UWB-based localization. In this paper, a ranging protocol is proposed that allows all robots to passively listen on neighbouring communicating robots without any hierarchical restrictions on the role of the robots. This is utilized to allow each robot to obtain more range measurements and to broadcast preintegrated inertial measurement unit (IMU) measurements for relative extended pose state estimation directly on SE2(3). Consequently, a simultaneous clock-synchronization and relative-pose estimator (CSRPE) is formulated using an on-manifold extended Kalman filter (EKF) and is evaluated in simulation using Monte-Carlo runs for up to 7 robots. The ranging protocol is implemented in C on custom-made UWB boards fitted to 3 quadcopters, and the proposed filter is evaluated over multiple experimental trials, yielding up to 48% improvement in localization accuracy.

==> sections/appx_approx_delta_t.tex <==
\jln{Under the approximation of constant clock skews during the TWR transaction shown on Figure \ref{fig:ds_twr},
we have
\begin{align*}
\Delta t^{21}_{f_0} &= T^2_{f_0} - R^1_{f_0} = T^2 + \tau_{f_o r}(T^2) - R^1 - \tau_{f_0 r}(R^1) \\
&= (1 + \gamma_{f_0 r}) \Delta t^{21}.
\end{align*}
Note that clock skews for typical commercial off-the-shelf electronic circuits if of the order
of parts-per-million \cite{Neirynck2017} and $\Delta t^{21}$ is in the order of hundreds of microseconds.
This justifies the approximation
\[
\gamma_{f_1 f_0} \Delta t^{21}_{f_0} = (\gamma_{f_1 f_0} + \gamma_{f_1 f_0} \gamma_{f_0 r}) \Delta t^{21} \approx \gamma_{f_1 f_0} \Delta t^{21}
\]
used in \eqref{eq:ts2}, by neglecting the terms of order $2$ in clock skew.
}
%The time interval $\Delta t^{21}$ in the ranging protocol shown in Figure \ref{fig:ds_twr} 
%is measured by the clock of Transceiver $s_2$,
\jln{Similarly, consider}
\begin{align*}
    \Delta \tilde{t}^{21}_{s_2} &= \tilde{\mathtt{T}}_{s_2}^{2} - \tilde{\mathtt{R}}_{s_2}^{1} \\
    % 
    &=  (1 + \gamma_{s_2 f_0}) \Delta t^{21}_{f_0} + \eta_{s_2}^{2} - \eta_{s_2}^{1}.
\end{align*}
However, given that the delay intervals in the passive-listening pseudomeasurements are only of the form $(\gamma_{i f_0} - \gamma_{s_2 f_0}) \Delta t^{21}_{f_0}$ and $(\gamma_{i f_0} - \gamma_{s_2 f_0}) \Delta t^{31}_{f_0}$, the approximation 
\begin{align*}
    (\gamma_{i f_0} - \gamma_{s_2 f_0}) \Delta \tilde{t}^{21}_{s_2} &= (\gamma_{i f_0} - \gamma_{s_2 f_0}) \Delta t^{21}_{f_0} \nonumber \\ &\hspace{12pt} + (\gamma_{i f_0} - \gamma_{s_2 f_0}) \gamma_{s_2 f_0} \Delta t^{21}_{f_0} \nonumber \\ &\hspace{12pt} + (\gamma_{i f_0} - \gamma_{s_2 f_0}) (\eta_{s_2}^{2} - \eta_{s_2}^{1}) \\
    %
    &\approx (\gamma_{i f_0} - \gamma_{s_2 f_0}) \Delta t^{21}_{f_0}
\end{align*}
can be made, and thus $(\gamma_{i f_0} - \gamma_{s_2 f_0})\Delta t^{21}_{f_0} \approx (\gamma_{i f_0} - \gamma_{s_2 f_0})\Delta \tilde{t}^{21}_{s_2} = (\gamma_{i f_0} - \gamma_{s_2 f_0})(\tilde{\mathtt{T}}_{s_2}^{2} - \tilde{\mathtt{R}}_{s_2}^{1})$. 
%This is due to the skew being typically in the order of parts-per-million \cite{Neirynck2017}, 
timestamping noise in the order of nanoseconds, 
%and $\Delta t^{21}$ in the order of hundreds of microseconds. 
Therefore, multiplying any skew terms with one another or with timestamping noise results 
in very small terms that are orders of magnitude smaller 
than $(\gamma_{i f_0} - \gamma_{s_2 f_0}) \Delta t^{21}_{f_0}$. 
The same analysis applies to $\Delta t^{31}$, which can likewise be approximated as
\beq
    (\gamma_{i f_0} - \gamma_{s_2 f_0})\Delta t^{31}_{f_0} \approx (\gamma_{i f_0} - \gamma_{s_2 f_0})(\tilde{\mathtt{T}}_{s_2}^{3} - \tilde{\mathtt{R}}_{s_2}^{1}). \nonumber
\eeq

==> sections/initialization.tex <==
\textcolor{red}{\#TODO: The initialization step when robots are static.}


==> sections/ranging_protocol_old.tex <==
\subsection{Overview}

\begin{figure}
    \centering
    \includegraphics[width=0.9\columnwidth]{figs/ranging_protocol/ds_twr.eps}
    \caption{%Schematic showing the 
    Proposed ranging protocol when Transceiver $f_1$ is initiating a DS-TWR ranging transaction with Transceiver $s_2$. This paper proposes that all other transceivers listen in on these \jln{messages}. Shown here are Transceivers $f_0$ and $s_0$ on Robot~0 passively listening, where the time instance corresponding to the $i^\text{th}$ passive reception at Transceiver $j$ is denoted $\mathtt{P}^{i,j}$.}
    \label{fig:ds_twr}
\end{figure}

To address the communication constraints, a ranging protocol is proposed that involves performing TWR between all pairs of transceivers not on the same robot in sequence while leveraging passive listening measurements at all other transceivers \jln{that are} not actively ranging. This is shown in Figure \ref{fig:ds_twr} for an example where Transceiver $f_1$ is initiating a TWR \jln{transaction} with transceiver $s_2$, and Transceivers $f_0$ and $s_0$ are passively listening. In the proposed ranging protocol, any of the $2(n+1)$ transceivers can initiate a TWR transaction with any of the $2n$ transceivers not on the same robot. 
%as the initiating one. 
In this section, the passive listening measurements are utilized in the relative-pose state estimator as a source of ranging information between the different robots. This is possible due to the tightly-coupled nature of the proposed estimator, which performs both clock synchronization and relative pose estimation, meaning that clock-offset-corrupted passive listening measurements can still be used to correct relative pose states, as cross-correlation information is available between clock states and relative pose states at all times.

There are multiple advantages to passive listening in multi-robot pose estimation applications, three of which are highlighted here.
\begin{enumerate}
    \item A $(1+3n)$-fold increase in the total number of distinct measurements when considering a centralized approach where passive listening measurements from all robots are available, and a $(\f{1}{2}+2n)$-fold increase in the number of distinct measurements when considering the perspective of an individual robot that does not have access to passive listening measurements at other robots. For example, for 5 neighbouring robots, this results in a 16-fold and an 11.5-fold increase in the number of measurements, respectively. The former is purely due to passive listening measurements, while the latter is due to passive listening measurements as well as the ability to obtain direct time-of-flight (ToF) measurements between two neighbouring robots. The proof of this claim is  given in Appendix \ref{appx:fold}.
    \item The ability to broadcast information such as IMU measurements or estimated maps at a higher rate as any robot can obtain information communicated between two neighbouring robots. This allows the use of multi-robot preintegration in Section \ref{sec:preint}.
    \item The ability to implement simple MAC protocols to schedule which pair will range next. Passive listening allows an alternative algorithm that combines the customizability of TDMA and the robustness of the \emph{token-passing protocol} \cite[Chapter 3.3]{miao2016}. Given that \jln{each} robot %now have access to the knowledge of 
    \jln{knows}
    which robots are currently ranging, a user-defined sequence of ranging pairs can be made known to all robots. Each robot can then keep track of which pair in the sequence is currently ranging, and initiate a TWR transaction to a specified transceiver when it is its turn to do so. This MAC protocol is named here the \emph{common-list protocol}, and has the advantage over the token-passing protocol that it allows more customizability on the sequence of ranging pairs without having to allocate discrete-time windows like in TDMA.
\end{enumerate}

When implementing the ranging protocol, a choice has to be made on the receiving robot's 
side (in this case, Robot~2) for the delays $\Delta t^{21} \coloneqq \mathtt{T}^{2} - \mathtt{R}^{1}$ and 
$\Delta t^{31} \coloneqq \mathtt{T}^{3} - \mathtt{R}^{1}$. 
% Notice that these values can be %recorded 
% \jln{resolved}
% in different clocks; for example, in clock $f_0$, 
% $\Delta t^{21}_{f_0} = \mathtt{T}^{2}_{f_0} - \mathtt{R}^{1}_{f_0}$. 
These user-defined parameters affect the frequency and noise of the measurements, 
and can be chosen based on \cite{Shalaby2022b}. 
We define also $\Delta t^{32} \coloneqq \Delta t^{31} - \Delta t^{21}$, 
and \jln{use a subscript to refer to these quantities resolved in a specific clock, e.g.,
$\Delta t^{21}_{f_0} \coloneqq \mathtt{T}^{2}_{f_0} - \mathtt{R}^{1}_{f_0}$}. 
Additionally, it will be assumed throughout this paper that the distances between 
transceivers and the clock skews remain constant during one ranging transaction. 
These are \jln{good} approximations for most robotic applications with %slowly-varying 
\jln{typical} clock rate \jln{variations} \cite[Chapter 7.1.4]{groves2013}, \cite{Shalaby2022b}. 

The remainder of this section analyzes how the proposed ranging protocol can be used in a CSRPE. The particular scenario under study is the one shown in Figures \ref{fig:ranging} and \ref{fig:ds_twr}, where transceivers on two neighbouring robots are the ones actively ranging. This is the most general case, and scenarios where one of the transceivers on Robot~0 is actively ranging \jln{involve} similar \jln{but simpler} derivations. %that are in fact slightly less involved. 
Note that in Figure \ref{fig:ds_twr}, all timestamps are available at Robot~0 \jln{at the end of
the transaction shown}, because the timestamps recorded at Robot~1 are communicated in the 
final information message shown in red and the timestamps recorded at Robot~2 are communicated 
in the last message transmitted by Robot~2. 

\subsection{\jln{Modelling} Timestamp \jln{Measurements}}

%The timestamps 
\jln{The time instances}
shown in Figure \ref{fig:ds_twr} are only available to the robots as noisy 
%measurements 
\jln{timestamps}
and in the clocks of the transceivers rather than in some global common time. 
Therefore, %these measurements 
\jln{the timestamp measurements}
are affected by clock offsets, clock skews, and white noise. 
Modelling these effects, \jln{with the offset definition in \eqref{eq: offset general definition}},
the timestamps available at Robot~1 (hereinafter, the \emph{initiating robot}) are of the form
\begin{align}
    \tilde{\mathtt{T}}_{f_1}^{1} &= \mathtt{T}_{f_0}^{1} + \tau_{f_1 f_0} + \eta_{f_1}^{1}, \label{eq:ts1}\\
    \tilde{\mathtt{R}}_{f_1}^{2} &= \mathtt{T}_{f_0}^{1} + \f{2}{c}d^{s_2 f_1} + \tau_{f_1 f_0} + (1 + \gamma_{f_1 f_0}) \Delta t^{21}_{f_0} + \eta_{f_1}^{2}, \label{eq:ts2} \\
    \tilde{\mathtt{R}}_{f_1}^{3} &= \mathtt{T}_{f_0}^{1} + \f{2}{c}d^{s_2 f_1} + \tau_{f_1 f_0} + (1 + \gamma_{f_1 f_0}) \Delta t^{31}_{f_0} + \eta_{f_1}^{3}, \label{eq:ts3}
\end{align}
where $\tilde{(\cdot)}$ here denotes a measured value, 
\jln{$\tau_{f_1 f_0}$ is the clock offset at time $T^1$},
$d^{s_2f_1}$ is the distance between Transceivers $s_2$ and $f_1$,
and $\eta_i^{\ell}$ is the random noise on the $\ell^\text{th}$ measurement of Transceiver $i$.
\jln{All the random noise variables are assumed to be independent, zero-mean and with the 
same variance $\sigma^2$.}
%and $\eta_i^{\ell} \sim \mc{N} (0, \sigma^2)$ is white Gaussian measurement noise associated with the %$\ell^\text{th}$ measurement of Transceiver $i$. 
Note that errors due to skew are considered during the delays $\Delta t^{21}$ and $\Delta t^{31}$ 
but not during the time of flight $\f{1}{c}d$, since $\Delta t^{21}, \Delta t^{31} \gg \f{1}{c}d$.
\jln{In addition, \eqref{eq:ts2}-\eqref{eq:ts3} use the approximations 
$\gamma_{f_1 f_0} \Delta t^{21} \approx \gamma_{f_1 f_0} \Delta t^{21}_{f_0}$
and $\gamma_{f_1 f_0} \Delta t^{31} \approx \gamma_{f_1 f_0} \Delta t^{31}_{f_0}$,
which are justified in Appendix \ref{appx:approx_delta_t}.}

Similarly, the measurements available at Robot~2 (hereinafter, the \emph{target robot}) are of the form
\begin{align}
    \tilde{\mathtt{R}}_{s_2}^{1} &= \mathtt{T}_{f_0}^{1} + \f{1}{c}d^{s_2 f_1} + \tau_{s_2 f_0} + \eta_{s_2}^{1}, \label{eq:ts4} \\
    \tilde{\mathtt{T}}_{s_2}^{2} &= \mathtt{T}_{f_0}^{1} + \f{1}{c}d^{s_2 f_1} + \tau_{s_2 f_0} + (1 + \gamma_{s_2 f_0}) \Delta t^{21}_{f_0} + \eta_{s_2}^{2}, \label{eq:ts5}\\
    \tilde{\mathtt{T}}_{s_2}^{3} &= \mathtt{T}_{f_0}^{1} + \f{1}{c}d^{s_2 f_1} + \tau_{s_2 f_0} + (1 + \gamma_{s_2 f_0}) \Delta t^{31}_{f_0} + \eta_{s_2}^{3}. \label{eq:ts6}
\end{align}

The timestamp measurements \eqref{eq:ts1}-\eqref{eq:ts6} correspond to the standard DS-TWR protocol, 
from which ToF pseudomeasurements can be generated. Nonetheless, additional measurements are available 
at Robot~0 (hereinafter, the \emph{passive robot}) since its transceivers $f_0$ and $s_0$ also receive 
the messages exchanged between the two actively ranging robots. 
This yields the following additional timestamp measurements at Robot~0,
\begin{align}
    \tilde{\mathtt{P}}_{i}^{1,i} &= \mathtt{T}_{f_0}^{1} + \f{1}{c}d^{f_1 i} + \tau_{i f_0} + \eta_{i}^{1}, \label{eq:ts7} 
\end{align}
\begin{align}
    \tilde{\mathtt{P}}_{i}^{2,i} &= \mathtt{T}_{f_0}^{1} + \f{1}{c}d^{s_2 f_1} + \f{1}{c}d^{f_1 i} + \tau_{i f_0} + (1 + \gamma_{i f_0}) \Delta t^{21}_{f_0} + \eta_{i}^{2}, \label{eq:ts8} \\
    \tilde{\mathtt{P}}_{i}^{3,i} &= \mathtt{T}_{f_0}^{1} + \f{1}{c}d^{s_2 f_1} + \f{1}{c}d^{f_1 i} + \tau_{i f_0} + (1 + \gamma_{i f_0}) \Delta t^{31}_{f_0} + \eta_{i}^{3}, \label{eq:ts9}
\end{align}
where $i \in \{ f_0, s_0 \}$ and $\tau_{f_0 f_0} = \gamma_{f_0 f_0} = 0$. 
Similarly, each neighbouring robot not involved in the ranging transaction records 
\jln{its} own passive listening measurements at its \jln{two} transceivers. 
However, these are not shared with other robots as this would require each robot 
to take its turn transmitting a message.

In the case where Robot~0 is not involved in the ranging transaction and just listens in passively, there are 12 available timestamp measurements at Robot~0, 6 sent by neighbouring robots, and 3 passive-listening timestamps per transceiver on Robot~0. However, when one of the transceivers $f_0$ or $s_0$ is involved in the ranging transaction, only 9 timestamp measurements are then available. Additionally, in the case where Transceiver $f_0$ is an active transceiver, the equations \eqref{eq:ts1}-\eqref{eq:ts6} are simpler as the clock states are being modelled relative to this transceiver. For example, if Transceiver $f_0$ initiates, the timestamp measurements \eqref{eq:ts1}-\eqref{eq:ts3} \jln{become}
\begin{align*}
    \tilde{\mathtt{T}}_{f_0}^{1} &= \mathtt{T}_{f_0}^{1} + \eta_{f_0}^{1},\\
    \tilde{\mathtt{R}}_{f_0}^{2} &= \mathtt{T}_{f_0}^{1} + \f{2}{c}d^{s_2 f_0} + \Delta t_{f_0}^{21} + \eta_{f_0}^{2}, \\
    \tilde{\mathtt{R}}_{f_0}^{3} &= \mathtt{T}_{f_0}^{1} + \f{2}{c}d^{s_2 f_0} + \Delta t_{f_0}^{31} + \eta_{f_0}^{3},
\end{align*}
where clock states no longer appear.

\subsection{Pseudomeasurements as a function of the state}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.3\columnwidth]{figs/ranging_protocol/known_vector.eps}
%     \caption{An example of the position of a transceiver relative to the IMU of Robot~0. Throughout this paper, it is assumed that the IMU is at the center of the robot.}
%     \label{fig:known_vector}
% \end{figure}

To use the timestamp measurements \eqref{eq:ts1}-\eqref{eq:ts9} in the CSRPE, they must be rewritten as a function of the state being estimated. In this subection, pseudomeasurements of the timestamps available at Robot 0 after one TWR transaction are formulated to get models that are only a function of the states being estimated, as well as the known vectors between the transceivers and the IMUs resolved in the robot's body frame.

First, notice that the distance $d^{s_2 f_1}$ between transceivers in \eqref{eq:ts1}-\eqref{eq:ts6} is a function of the states, and can be written as 
\begin{align}
    d^{s_2 f_1} &= \norm{\mbf{r}_0^{s_2 f_1}} \nonumber \\
    %
    &= \norm{\mbf{r}_0^{s_2 0} - \mbf{r}_0^{f_1 0}} \nonumber \\
    % 
    &= \norm{(\mbf{C}_{02} \mbf{r}_2^{s_2 2} + \mbf{r}_0^{2 0}) - (\mbf{C}_{01} \mbf{r}_1^{f_1 1} + \mbf{r}_0^{1 0})} \nonumber \\
    %
    &= \norm{\mbftilde{1} \left(\mbf{T}_{02} \mbftilde{r}_2^{s_2 2} - \mbf{T}_{01} \mbftilde{r}_1^{f_1 1} \right)}, \label{eq:dist}
\end{align}
where $\norm{\cdot}$ is the Euclidean norm, $\mbftilde{1} = \bma{ccc} \mbf{1}_3 & \mbf{0}_3 & \mbf{0}_3 \ema \in \mathbb{R}^{3 \times 9}$, and
\beq
    \mbftilde{r} = \bma{ccc} 
        \mbf{r}^\trans & 0 & 1
    \ema^\trans. \nonumber
\eeq
For an EKF, the linearization of \eqref{eq:dist} with respect to the state is shown in Appendix \ref{appx:linearize_range}.

Therefore, pseudomeasurements can be generated that are only a function of the distance between the transceivers, the clock states, and the white noise. The \textbf{first pseudomeasurement} is the standard ToF measurement associated with DS-TWR \cite{Shalaby2022a}, which from timestamps \eqref{eq:ts1}-\eqref{eq:ts6} can be written as
\begin{align}
    y^\text{tof} &= \f{1}{2} \left( \left( \tilde{\mathtt{R}}_{f_1}^{2} - \tilde{\mathtt{T}}_{f_1}^{1} \right) - \f{\tilde{\mathtt{R}}_{f_1}^{3} - \tilde{\mathtt{R}}_{f_1}^{2}}{\tilde{\mathtt{T}}_{s_2}^{3} - \tilde{\mathtt{T}}_{s_2}^{2}} \left( \tilde{\mathtt{T}}_{s_2}^{2} - \tilde{\mathtt{R}}_{s_2}^{1} \right) \right) \nonumber \\
    %
    &\approx \f{1}{c} d^{s_2 f_1} + \f{1}{2} \left( \eta_{f_1}^{2} - \eta_{f_1}^{1} + \eta_{s_2}^{2} - \eta_{s_2}^{1} \right), \label{eq:y_r}
\end{align}
where the approximations 
\beq
    \f{(1 + \gamma_{f_1 f_0}) \Delta t^{32}_{f_0} + \eta_{f_1}^{3} - \eta_{f_1}^{2}}{(1 + \gamma_{s_2 f_0}) \Delta t^{32}_{f_0} + \eta_{s_2}^{3} - \eta_{s_2}^{2}} \approx \f{(1 + \gamma_{f_1 f_0})}{(1 + \gamma_{s_2 f_0})} \nonumber
\eeq
and
\beq
    \f{(1 + \gamma_{f_1 f_0})}{(1 + \gamma_{s_2 f_0})} \left( \eta_{s_2}^{2} - \eta_{s_2}^{1} \right) \approx \eta_{s_2}^{2} - \eta_{s_2}^{1} \nonumber
\eeq
are made. The first approximation follows from an assumption that typically $\Delta t^{32}$, which is in the order of hundreds of microseconds or milliseconds, is significantly bigger than the timestamping noise, which is in the order of a few hundred picoseconds at most. The second approximation, which simplifies the derivation significantly, follows from the fact that the clock skew and timestamping noise are small.

The \textbf{second pseudomeasurement} is a direct clock offset measurement between the initiating and target transceivers, which from timestamps \eqref{eq:ts1}-\eqref{eq:ts6} can be written as
\begin{align}
    y^\tau &= \f{1}{2} \left( \left( \tilde{\mathtt{R}}_{f_1}^{2} + \tilde{\mathtt{T}}_{f_1}^{1} \right) - \f{\tilde{\mathtt{R}}_{f_1}^{3} - \tilde{\mathtt{R}}_{f_1}^{2}}{\tilde{\mathtt{T}}_{s_2}^{3} - \tilde{\mathtt{T}}_{s_2}^{2}} \left( \tilde{\mathtt{T}}_{s_2}^{2} - \tilde{\mathtt{R}}_{s_2}^{1} \right) - 2\tilde{\mathtt{R}}_{s_2}^{1} \right) \nonumber \\
    %
    &\approx \tau_{f_1 f_0} - \tau_{s_2 f_0} + \f{1}{2} \left( \eta_{f_1}^{2} + \eta_{f_1}^{1} - \eta_{s_2}^{2} - \eta_{s_2}^{1} \right). \label{eq:y_tau}
\end{align}
This is somewhat similar to the measurement model proposed in \cite{Cano2019}, but involves an additional term to correct the effect of the clock skew on the measured offset. 

The \textbf{third pseudomeasurement} is associated with the first passive-listening timestamp, which is a function of the distance between the passive robot and the initiating robot, as well the clock offset between the two transceivers. Using timestamps \eqref{eq:ts1} and \eqref{eq:ts7} for $i \in \{f_0, s_0\}$, this is written as
\begin{align}
    y^\text{p,1}_{i} &= \tilde{\mathtt{P}}_{i}^{1,i} - \tilde{\mathtt{T}}_{f_1}^{1} \nonumber \\
    %
    &= \f{1}{c}d^{f_1 i} + \tau_{i f_0} - \tau_{f_1 f_0} + \eta_{i}^{1} - \eta_{f_1}^{1}.
    \label{eq:y_p1}
\end{align}

The \textbf{fourth pseudomeasurement} is similar to the third one, with an additional skew-correction component to model the passage of time $\Delta t^{21}$ between the first and second signal in two clocks with different clock rates. Using timestamps \eqref{eq:ts5} and \eqref{eq:ts8} for $i \in \{f_0, s_0\}$ , this is modelled as
\begin{align}
    y^\text{p,2}_{i} &= \tilde{\mathtt{P}}_{i}^{2,i} - \tilde{\mathtt{T}}_{s_2}^{2} \nonumber \\
    %
    &= \f{1}{c}d^{f_1 i} + \tau_{i f_0} - \tau_{s_2 f_0} \nonumber \\ &\hspace{30pt} + (\gamma_{i f_0} - \gamma_{s_2 f_0}) \Delta t^{21}_{f_0} + \eta_{i}^{2} - \eta_{s_2}^{2} \label{eq:y_p2}
\end{align}

Lastly, the \textbf{fifth pseudomeasurement} is similar to the fourth pseudomeasurement, but modelling the evolution of the clocks over a longer time window $\Delta t^{31}$. Using timestamps \eqref{eq:ts6} and \eqref{eq:ts9} for $i \in \{f_0, s_0\}$, this is modelled as
\begin{align}
    y^\text{p,3}_{i} &= \tilde{\mathtt{P}}_{i}^{3,i} - \tilde{\mathtt{T}}_{s_2}^{3} \nonumber \\
    %
    &= \f{1}{c}d^{f_1 i} + \tau_{i f_0} - \tau_{s_2 f_0} \nonumber \\ &\hspace{30pt} + (\gamma_{i f_0} - \gamma_{s_2 f_0}) \Delta t^{31}_{f_0} + \eta_{i}^{3} - \eta_{s_2}^{3}. \label{eq:y_p3}
\end{align}

Note the last three pseudomeasurements are per listening transceiver $i$, and therefore there are a total of 8 pseudomeasurements available at Robot~0 if it is not involved in the ranging transaction, or 5 pseudomeasurements if one of the transceivers on Robot~0 is active.

Additionally, note that the delay intervals $\Delta t^{21}$ and $\Delta t^{31}$ appear in the pseudomeasurements \eqref{eq:y_p2}-\eqref{eq:y_p3} as if the length of the interval is known in the clock of Transceiver $f_0$. These are in fact unknown values, as the delay values are programmed into all transceivers manually, which then enforce these delays in their own clocks, so in the scenario presented in Figure \ref{fig:ds_twr} the only measured values are $\Delta t^{21}_{s_2}$ and $\Delta t^{31}_{s_2}$. Nonetheless, the approximation
\begin{align*}
    (\gamma_{i f_0} - \gamma_{s_2 f_0})\Delta t^{21}_{f_0} &\approx (\gamma_{i f_0} - \gamma_{s_2 f_0})(\tilde{\mathtt{T}}_{s_2}^{2} - \tilde{\mathtt{R}}_{s_2}^{1}), \\
    (\gamma_{i f_0} - \gamma_{s_2 f_0})\Delta t^{31}_{f_0} &\approx (\gamma_{i f_0} - \gamma_{s_2 f_0})(\tilde{\mathtt{T}}_{s_2}^{3} - \tilde{\mathtt{R}}_{s_2}^{1})
\end{align*}
can be made as explained in Appendix \ref{appx:approx_delta_t}.

\subsection{Cross-correlation between pseudomeasurements}

Given that the pseudomeasurements are a function of the same measured timestamps, cross-correlations between the pseudomeasurements exist and must be correctly modelled in the filter. Computing the variance of the pseudomeasurements \eqref{eq:y_r}-\eqref{eq:y_p3} is straightforward, and can be summarized as
\begin{align*}
    \mathbb{E}\left[ (y^\text{tof} - \bar{y}^\text{tof})^2 \right] &= \sigma^2, \\
    \mathbb{E}\left[ (y^\tau - \bar{y}^\tau)^2 \right] &= \sigma^2, \\
    \mathbb{E}\left[ (y^\text{p,j}_i - \bar{y}^\text{p,j}_i)^2 \right] &= 2\sigma^2, \quad j \in \{1,2,3\},
\end{align*}
where an overbar denotes a noise-free value. Meanwhile, the cross-correlation between the ToF and offset measurements can be computed as
\begin{align*}
    \mathbb{E}\left[ (y^\text{tof} - \bar{y}^\text{tof})(y^\tau - \bar{y}^\tau) \right] = 0
\end{align*}
as the noise values are of alternating signs. Lastly, the cross-correlation between the passive listening measurements and the ToF measurements can be shown to be
\begin{align*}
    \mathbb{E}\left[ (y^\text{p,1}_i - \bar{y}^\text{p,1}_i)(y^\text{tof} - \bar{y}^\text{tof}) \right] &= \sigma^2, \\
    \mathbb{E}\left[ (y^\text{p,2}_i - \bar{y}^\text{p,2}_i)(y^\text{tof} - \bar{y}^\text{tof}) \right] &= -\sigma^2, \\
    \mathbb{E}\left[ (y^\text{p,3}_i - \bar{y}^\text{p,3}_i)(y^\text{tof} - \bar{y}^\text{tof}) \right] &= 0,
\end{align*}
while the cross-correlations with offset measurements are the same but with opposite signs. Passive listening measurements of different transceivers are also correlated. Stacking all the pseudomeasurements into one column matrix gives the measurement vector 
\beq
    \mbf{y} = \bma{cccccccc} y^\text{tof} & y^\tau & y^\text{p,1}_{f_0} & y^\text{p,2}_{f_0} & y^\text{p,3}_{f_0} & y^\text{p,1}_{s_0} & y^\text{p,2}_{s_0} & y^\text{p,3}_{s_0} \ema^\trans, \label{eq:meas}
\eeq
and the random measurement is distributed as per $\mbf{y} \sim \mc{N} (\mbfbar{y}, \mbf{R})$, where
\beq
    \mbf{R} = \bma{ccc}
        \sigma^2 \mbf{1}_2 & \f{1}{2} \sigma^2 \mbf{B} & \f{1}{2} \sigma^2 \mbf{B} \\
        \f{1}{2} \sigma^2 \mbf{B}^\trans & 2\sigma^2 \mbf{1}_3 & \sigma^2 \mbf{1}_3  \\
        \f{1}{2} \sigma^2 \mbf{B}^\trans & \sigma^2 \mbf{1}_3 & 2\sigma^2 \mbf{1}_3
    \ema, \nonumber
\eeq
and   
\beq
    \mbf{B} = \bma{ccc}
        1 & -1 & 0 \\
        -1 & 1 & 0
    \ema. \nonumber
\eeq
The measurement vector $\mbf{y}$ and its covariance $\mbf{R}$ are used in the correction step of an on-manifold EKF, where they are fused with the process model derived in the next section.
